Near Optimal Linear Algebra in the Online and Sliding Window Models

We initiate the study of numerical linear algebra in the sliding window model, where only the most recent $W$ updates in a stream form the underlying data set. We first introduce a unified row-sampling based framework that gives randomized algorithms for spectral approximation, low-rank approximation/projection-cost preservation, and $\ell_1$-subspace embeddings in the sliding window model, which often use nearly optimal space and achieve nearly input sparsity runtime. Our algorithms are based on "reverse online" versions of offline sampling distributions such as (ridge) leverage scores, $\ell_1$ sensitivities, and Lewis weights to quantify both the importance and the recency of a row. Our row-sampling framework rather surprisingly implies connections to the well-studied online model; our structural results also give the first sample optimal (up to lower order terms) online algorithm for low-rank approximation/projection-cost preservation. Using this powerful primitive, we give online algorithms for column/row subset selection and principal component analysis that resolves the main open question of Bhaskara et. al.,(FOCS 2019). We also give the first online algorithm for $\ell_1$-subspace embeddings. We further formalize the connection between the online model and the sliding window model by introducing an additional unified framework for deterministic algorithms using a merge and reduce paradigm and the concept of online coresets. Our sampling based algorithms in the row-arrival online model yield online coresets, giving deterministic algorithms for spectral approximation, low-rank approximation/projection-cost preservation, and $\ell_1$-subspace embeddings in the sliding window model that use nearly optimal space.

==> matrix-mult.tex <==
%!TEX root = randNLA-sliding.tex
\section{Covariance Matrix Approximation}
\seclab{sec:matrix-mult}
In this section, we describe how our downsampling procedure can be applied as a subroutine to perform covariance matrix approximation in the sliding window model. 
Given a data stream of elements $\r_1,\r_2,\ldots,\r_n\in\mathbb{R}^d$ be a stream of rows and $W$ be the size of the sliding window. 
Let $\A=\r_{n-W+1}\circ\ldots\circ\r_n$ be the matrix consisting of the $W$ most recent rows. 
Then the goal is to estimate the entries of $\A^\top\A$. 
We also point out that a similar algorithm and analysis handles approximate matrix multiplication in the sliding window model, where the columns of $\A\in\mathbb{R}^{m\times W}$ and the rows of $\B\in\mathbb{R}^{W\times p}$ arrive in sync, and the goal is to estimate $\A\B$. 

\subsection{Preliminaries}
In the classical offline model, $\A^\top\A$ can be estimated by sampling a fixed number of rows of $\A=\a_1\circ\ldots\circ\a_n$ to obtain a matrix $\B$ with
\[\EEx{\norm{\A^\top\A-\B^\top\B}_F}\le\eps\norm{\A}^2_F.\]
Each row of $\B$ is a sampled to row $\a_k$ of $\A$ with probability $p_k=\frac{\norm{\a_k}_2^2}{\norm{\A}_F^2}$ and then rescaled by $\frac{1}{\sqrt{p_k}}$. 
Since the number of rows of $\B$ is fixed, this approach can be viewed as a reservoir sampling paradigm. 

Instead of the reservoir sampling approach, we iterate through each of the rows of $\A$ and sample each row independently. 
We show that by sampling each row with probability roughly $p_k\ge\frac{c\cdot\norm{\a_k}_2^2}{\norm{\A}_F^2}$ for some fixed constant $c$ and then rescaling the row by $\frac{1}{\sqrt{p_k}}$ to form a matrix $\B$, then $\B^\top\B$ is a good approximation to $\A^\top\A$. 
The following result essentially follows the same proof as Theorem 22 in \cite{DrineasM17}. 
\begin{lemma}
\lemlab{lem:mm:ex}
If each row $\a_k$ of $\A$ is sampled with some probability $p_k$, where $p_k\ge\min\left(1,\frac{c\cdot\norm{\a_k}_2^2}{\norm{\A}_F^2}\right)$ for some fixed constant $c$ and all $1\le k\le n$, and then rescaled by $\frac{1}{\sqrt{p_k}}$ to obtain matrix $\B$, then
\[
\EEx{\norm{\A^\top\A-\B^\top\B}_F^2}\le\frac{1}{c}\norm{\A}_F^4.
\]
\end{lemma}
\begin{proof}
Observe that the expected value of each entry of $\B^\top\B$ is the value of the corresponding entry of $\A^\top\A$. 
\[\EEx{(\B^\top\B)_{i,j}}=\sum_{k=1}^n p_k\left(\frac{1}{p_k}\a_k^\top\a_k\right)_{i,j}=(\A^\top\A)_{i,j}.\] 
Moreover, the variance of each entry of $\B^\top\B$ can be bounded by
\[\var{(\B^\top\B)_{i,j}}\le\sum_{k=1}^n\frac{1}{p_k}(\a_k^\top\a_k)_{i,j}^2=\sum_{k=1}^n\frac{1}{p_k}(\A_{k,i}\A_{k,j})^2.\]
Since $\B^\top\B$ is an unbiased estimator of $\A^\top\A$, then
\begin{align*}
\EEx{\norm{\B^\top\B-\A^\top\A}_F^2}&=\sum_{i=1}^n\sum_{j=1}^n\EEx{\left(\A^\top\A-\B^\top\B\right)^2_{i,j}}\\
&=\sum_{i=1}^n\sum_{j=1}^n\var{\left(\A^\top\A-\B^\top\B\right)_{i,j}}\\
&\le\sum_{i=1}^n\sum_{j=1}^n\sum_{k=1}^n\frac{1}{p_k}(\A_{k,i}\A_{k,j})^2\\
&=\sum_{k=1}^n\frac{1}{p_k}\left(\sum_{i=1}^n\A_{k,i}^2\right)\left(\sum_{j=1}^n\A_{k,j}^2\right)\\
&=\sum_{k=1}^n\frac{1}{p_k}\norm{\a_k}_2^4.
\end{align*}
Hence for $p_k\ge\min\left(1,\frac{c\norm{\a_k}_2^2}{\norm{\A}_F^2}\right)$,
\[\EEx{\norm{\B^\top\B-\A^\top\A}_F^2}\le\frac{1}{c}\left(\sum_{j=1}^n\norm{\a_j}_F^2\right)\cdot\norm{\A}_F^2=\frac{1}{c}\norm{\A}_F^4.\]
\end{proof}

We cannot maintain $\norm{\A}_F^2$ in the sliding window model without using prohibitive space. 
However, using the \emph{smoothness} of the Frobenius norm, we can instead maintain a $2$-approximation of $\norm{\A}_F^2$ so that we can maintain ${\widehat p_t}$ to be a $2$-approximation of $p_t$. 
\begin{lemma}[Lemma 5 in \cite{BravermanO07}]
\lemlab{lem:frobenius:smooth}
The Frobenius norm is $\left(\eps,\frac{\eps^2}{4}\right)$-smooth. 
\end{lemma}
Recall from \appref{sec:smooth-histogram} that smooth functions can be well-approximated in the sliding window model. 

\subsection{Algorithm}
Each time an update arrives, we add the new rows to our samples. 
We then downsample each existing sampled row so that at the end of the stream, the probability we keep row $i$ is roughly proportional to $\frac{18}{\eps^2}\frac{\norm{\r_i}^2_2}{\widehat{f}}$, where $\widehat{f}$ is a $2$-approximation to the Frobenius norm of the matrix represented by the sliding window. 
We give the algorithm in full in \matrixmult{} (\algref{fig:mm:sample}). 
Like our previous sliding window algorithms, \matrixmult{} outputs the union of the rows in all the stored matrices as the covariance approximation to the underlying matrix since each matrix stored by \matrixmult{} only contains the rows that arrive \emph{between} two timestamps.

\begin{algorithm}[t]
\caption{\matrixmult: Covariance matrix approximation on sliding windows}
\alglab{fig:mm:sample}
\begin{algorithmic}[1]
\Require{A stream of rows $\r_1,\ldots,\r_n\in\mathbb{R}^d$, a parameter $W$ for the size of the sliding window, an accuracy parameter $\eps$.}
\Ensure{$(1+\eps)$-covariance matrix approximation in the sliding window model.}
%\State{$\M_1=0^{1\times n}, t_1=0, g_1=0$.}
\State{$\H\leftarrow\{\emptyset,\emptyset,\emptyset\}$.}
\For{each row $\r_t$}
\State{$\H\leftarrow\multupdate(\H,\r_t,t,\eps)$}
\State{$\H\leftarrow\multcompress(\H)$}
\State{$\H\leftarrow\multexpire(\H,t,W)$}
\EndFor
\State{$\M\leftarrow\emptyset$}
\For{$j=1$ to $j=s$, where $s$ is the number of matrices in $\H$}
\For{each row $\r_i\in\M_j$ in $\H$}
\State{$\M\leftarrow\M\circ\frac{1}{\sqrt{p_i}}\r_i$}
\Comment{Rescale output matrix by sampling probabilities}
\EndFor
\EndFor
\State{\Return $\M$.}
\end{algorithmic}
\end{algorithm}



\begin{algorithm}[!htb]
\caption{$\multupdate(\H,\r_t,t,\eps)$}
\alglab{alg:mult:update}
\begin{algorithmic}[1]
\Require{Data structure $\H$ consisting of matrices $\M_1,\ldots,\M_s$ with corresponding timestamps $t_1,\ldots,t_s$ and values $g_1,\ldots,g_s$ such that $g_i=\sum_{j=t_i}^t{\norm{\r_j}^2_2}$, row vector $\r_t\in\mathbb{R}^d$, current timestamp $t$, and accuracy parameter $\eps$. 
Each matrix has some stored row(s) $\r_i\in\mathbb{R}^{1\times n}$, each with an associated value $p_i$ and timestamp $i$. 
}
\Ensure{Updated data structure $\H$.}
\State{$c\leftarrow\frac{18}{\eps^2}$, $p_t\leftarrow c$}
\State{$\M_{s+1}\leftarrow\r_t$, $t_{s+1}\leftarrow t$, $g_{s+1}\leftarrow\norm{\r_t}^2_2$}
\Comment{Also store timestamp $t$ and associated probability $p_t$}
\For{$j=1$ to $j=s$}
\State{$g_j\leftarrow g_j+g_{s+1}$}
\Comment{Update Frobenius norm}
\For{each row $\r_k$ in $\M_j$}
\State{$q_k=\frac{g_j-g_{s+1}}{g_j}\cdot p_k$}
\Comment{Update downsampling probability}
\If{$q_k<1$}
\State{With probability $1-\frac{q_k}{\min(p_k,1)}$, delete $\r_k$ from $\M_j$}
\Comment{Downsample}
\EndIf
\State{$p_k\leftarrow q_k$}
\EndFor
%\WHILE{$\min\left(p_t\cdot\frac{g_{s+1}}{g_j},1\right)$}
%\State{$\M_j\leftarrow\M_j\cdot\r_t$}
%\Comment{Also store timestamp $t$ and associated probability}
%\ENDWHILE
\EndFor
\State{$s\leftarrow s+1$.}
\Return $\H$.
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[!htb]
\caption{$\multcompress(\H)$}
\alglab{alg:mult:compress}
\begin{algorithmic}[1]
\Require{Data structure $\H$ consisting of matrices $\M_1,\ldots,\M_s$ with corresponding timestamps $t_1,\ldots,t_s$ and values $g_1,\ldots,g_s$ such that $g_i=\sum_{j=t_i}^t{\norm{\r_j}^2_2}$, row vector $\r_t\in\mathbb{R}^d$, and current timestamp $t$. 
Each matrix has some stored row(s) $\r_i\in\mathbb{R}^{1\times n}$, each with an associated value $p_i$ and timestamp $i$. 
}
\Ensure{Updated data structure $\H$.}
\For{$i=1,\ldots, s-2$}
\State{Compute $j=\underset{k>i}{\max}\{k\,:\, g_k\ge\frac{1}{2} g_i\}$.}
\If{$j>i+1$}
\For{$k=i+1$ to $s-j+i+2$}
\For{each row $\r_\ell$ in $\M_k$}
\State{$q_\ell=\frac{g_k}{g_i}\cdot p_\ell$}
\Comment{Update downsampling probability}
\If{$q_k<1$}
\State{With probability $\frac{q_\ell}{\min(p_\ell,1)}$, $\M_j\leftarrow\M_j\circ\r_\ell$}
\Comment{Downsample}
\EndIf
\State{$p_\ell\leftarrow q_\ell$}
\EndFor
\EndFor
\State{Delete $\M_{i+1},\ldots,\M_{j-1}$ and $t_{i+1},\ldots,t_{j-1}$.}
\For{$k=i+1$ to $s-j+i+2$}
\State{$\M_k\leftarrow\M_{j-i+k-1}$}\Comment{Reorder indices.}
\State{$t_k\leftarrow t_{j-i+k-1}$}
\EndFor
\State{$s\leftarrow s-j+i+1$.}
\EndIf
\EndFor
\State{\Return $\H$.}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[!htb]
\caption{$\multexpire(\H,t,W)$}
\alglab{alg:mult:expire}
\begin{algorithmic}[1]
\Require{Data structure $\H$ consisting of matrices $\M_1,\ldots,\M_s$ with corresponding timestamps $t_1,\ldots,t_s$ and values $g_1,\ldots,g_s$ such that $g_i=\sum_{j=t_i}^t{\norm{\r_j}^2_2}$, row vector $\r_t\in\mathbb{R}^d$, current timestamp $t$, and window size $W$.}
\Ensure{Updated data structure $\H$.}
\For{row $\r_j$ in $\M_1$}
\If{$j\le t-W+1$}
\Comment{If row is expired.}
\State{Delete $\r_j$.}
\EndIf
\EndFor
\If{$t_2\le t-W+1$}
\Comment{If second timestamp is expired.}
\State{Delete $\M_1$ and $t_1$.}
\For{$k=1$ to $s$}
\State{$\a_k\leftarrow\a_{k+1}$}\Comment{Reorder indices.}
\State{$t_k\leftarrow t_{k+1}$}
\EndFor
\State{$s\leftarrow s-1$.}
\EndIf
\State{\Return $\H$.}
\end{algorithmic}
\end{algorithm}

We first show that each row $\r_i$ in $\A$ is sampled with probability roughly $\frac{\norm{\r_i}_2^2}{\norm{\A}_F^2}$, where $\A$ is the matrix represented by the sliding window. 
Intuitively, upon the arrival of each new row, each previous row $\r_j$ is downsampled in \multupdate{} with probability that equals the relative change of the Frobenius norm. 
Specifically, if $g_j$ is the Frobenius norm of the rows $\r_j\circ\ldots\circ\r_t$, then $\r_j$ is retained with probability $\frac{g_j}{g_j-\norm{\r_t}_2^2}$, which is the relative change of the Frobenius norm. 
Similarly, when two sketches are compressed in \multcompress, $\r_j$ is downsampled with probability that equals the ratio of the Frobenius norm of the matrices represented by the sketches. 
That is, when sketch $k$ is merged with sketch $j$, then a row $\r_i$ in sketch $k$ is retained with probability $\frac{g_k}{g_j}$, which is the ratio of the Frobenius norm of the matrices represented by the sketches. 
Hence, the probability that $\r_j$ is retained at the end of the stream is roughly the ratio $\norm{\r_j}_F^2$ (scaled by $c$) to the Frobenius norm of the final sketch, $p_j=\frac{18}{\eps^2}\frac{\norm{\r_j}^2_2}{\norm{\A_i}_F^2}$.
\begin{lemma}
\lemlab{lem:mm:sample:prob}
For a row $\r_j$ where $j\ge t-W+1$, let $t_i\le j<t_{i+1}$ and $\A_i=\r_{t_i}\circ\ldots\circ\r_t$. 
Then each row $\r_j$ is sampled in \algref{fig:mm:sample} with probability $p_j=\min\left(1,\frac{18}{\eps^2}\frac{\norm{\r_j}^2_2}{\norm{\A_i}_F^2}\right)$. 
\end{lemma}
\begin{proof}
We give a proof by induction, observing for the base case that the newest row is always sampled by \multupdate. 
Prior to the arrival of row $\r_t$, let the rows stored by \algref{fig:mm:sample} be $\a_1,\ldots,\a_s$ and suppose $t_k\le j<t_{k+1}$. 
Let $\A_k=\r_{t_k}\circ\ldots\circ\r_{t-1}$ and suppose the probability that row $\r_j$ is sampled is $\min\left(1,\frac{18}{\eps^2}\frac{\norm{\r_j}^2_2}{\norm{\A_k}_F^2}\right)$. 
Upon the arrival of row $\r_t$, \multupdate{} first computes the probability $\frac{g_k-g_{s+1}}{g_k}=\frac{\norm{\A_k}_F^2}{\norm{\A_k}_F^2+\r_t^2}$. 
Hence for each row $\r_j$, we have $p_j=\frac{18}{\eps^2}\frac{\norm{\r_j}^2_2}{\norm{\A_k}_F^2+\r_t^2}$, so row $\r_j$ is sampled with probability $\min\left(1,\frac{18}{\eps^2}\frac{\norm{\r_j}^2_2}{\norm{\A_k}_F^2+\r_t^2}\right)$. 
However if $\A_k$ is not deleted by \multcompress, then $\norm{\A_k}_F^2+\r_t^2$ is just the definition of $\norm{\A_i}_F^2$ after the arrival of row $\r_t$ in the statement of \lemref{lem:mm:sample:prob}. 

On the other hand, if $\A_k$ is deleted by \multcompress, then $\r_j$ is downsampled by \multcompress{} with probability $\frac{g_i}{g_k}=\frac{\norm{\A_i}_F^2}{\norm{\A_k}_F^2+\r_t^2}$, where $\A_i$ is the updated Frobenius norm after the arrival of row $\r_t$. 
Hence the same argument applies, so row $\r_j$ is sampled with probability $\min\left(1,\frac{18}{\eps^2}\frac{\norm{\r_j}^2_2}{\norm{\A_i}_F^2}\right)$, and the induction is complete.  
\end{proof}

We now justify the correctness and space complexity of \algref{fig:mm:sample}.
\begin{theorem}
\thmlab{thm:matrixmult:words}
Let $\r_1,\ldots,\r_n\in\mathbb{R}^d$ be a stream of rows and $W$ be the size of the sliding window. 
Let $\A=\r_{n-W+1}\circ\ldots\circ\r_n$ be the matrix consisting of the $W$ most recent rows. 
Then given a parameter $\eps>0$, there exists an algorithm that, with probability at least $\frac{2}{3}$, outputs a matrix $\B$ with a subset of (rescaled) rows of $\A$ such that
\[\norm{\A^\top\A - \B^\top\B}_F\le\eps\norm{\A}^2_F.\]
With high probability, the algorithm uses $\O{\frac{d}{\eps^2}\log^2 n}$ space.
\end{theorem}
\begin{proof}
Let $t_1,\ldots,t_s$ be the timestamps maintained by \algref{fig:mm:sample} and $\A_1=\r_{t_1}\circ\cdots\circ\r_n$. 
By construction, the sequence $g_1,\ldots,g_s$ corresponds exactly to a smooth histogram that computes a $2$-approximation to the Frobenius norm (see \appref{sec:smooth-histogram} for example). 
Thus by \lemref{lem:frobenius:smooth} and the properties of the smooth histogram, $\norm{\A_1}^2_F\le 2\norm{\A}^2_F$. 
Hence by \lemref{lem:mm:sample:prob}, each row $\a_i$ in $\A$ is sampled with probability at least $\frac{9}{\eps^2}\frac{\norm{\a_i}^2_2}{\norm{\A}_F^2}$.
From \lemref{lem:mm:ex}, it follows that
\[
\EEx{\norm{\A^\top\A-\B^\top\B}_F^2}\le\frac{\eps^2}{9}\norm{\A}^4_F.
\]
Then by Jensen's inequality,
\[
\EEx{\norm{\A^\top\A-\B^\top\B}_F}\le\sqrt{\EEx{\norm{\A^\top\A-\B^\top\B}_F^2}}\le\frac{\eps}{3}\norm{\A}^2_F.
\]
A standard application of Markov's inequality gives the desired result for correctness. 

To analyze the space complexity, first observe that $s=\O{\log n}$ since we only require a $2$-approximation to the Frobenius norm, and a separate matrix is associated with each instance in the smooth histogram. 
Then by a simple Chernoff bound and the observation that $c=\O{\frac{1}{\eps^2}}$, it follows that \matrixmult{} stores $\O{\frac{1}{\eps^2}\log n}$ rows, with high probability, each with dimension $d$. 
Therefore, \matrixmult{} uses $\O{\frac{d}{\eps^2}\log^2 n}$ bits of space.
\end{proof}
We observe that by rounding the entries in each stored row after the sampling probabilities are computed, we can avoid using $\O{d\log n}$ space per row.
\begin{theorem}
\thmlab{thm:matrixmult:bits}
Let $\r_1,\ldots,\r_n\in\mathbb{R}^d$ be a stream of rows and $W$ be the size of the sliding window. 
Let $\A=\r_{n-W+1}\circ\ldots\circ\r_n$ be the matrix consisting of the $W$ most recent rows. 
Then given a parameter $\eps>0$, there exists an algorithm that, with probability at least $\frac{2}{3}$, outputs a matrix $\B$ with a subset of (rescaled) rows of $\A$ such that
\[\norm{\A^\top\A - \B^\top\B}_F\le\eps\norm{\A}^2_F.\]
With high probability, the algorithm uses $\O{\frac{d}{\eps^2}\log n\left(\log\log n+\log\frac{1}{\eps}\right)}$ space.
\end{theorem}
\begin{proof}
Given a matrix $\A$, we round each nonzero entry of $\A$ to the closest power of $\left(1+\frac{\eps}{6}\right)$ to form a matrix $\C$. 
Then $\left(1-\frac{\eps}{6}\right)\A_{i,j}\le\C_{i,j}\le\left(1+\frac{\eps}{6}\right)\A_{i,j}$. 
Hence, we can write $\A=\C+\bD$ for some matrix $\bD$ where $|\bD_{i,j}|\le\frac{\eps}{6}|\A_{i,j}|$. 
Thus,
\begin{align*}
\norm{\A^\top\A-\C^\top\C}_F&=\norm{\C^\top\bD+\bD^\top\C+\bD^\top\bD}_F\\
&\le\norm{\C^\top\bD}_F+\norm{\bD^\top\C}_F+\norm{\bD^\top\bD}_F\\
&\le2\norm{\C}_F\norm{\bD}_F+\norm{\bD}^2_F\\
&\le\left(2+\frac{\eps}{3}+\frac{\eps}{6}\right)\frac{\eps}{6}\norm{\A}^2_F\\
&<\frac{\eps}{2}\norm{\A}^2_F,
\end{align*}
for $\eps<1$. 

By sending the rows of $\C$ into \matrixmult{} with approximation parameter $\frac{\eps}{8}$, the output matrix $\B$ satisfies
\[\norm{\C^\top\C-\B^\top\B}\le\frac{\eps}{8}\norm{\C}^2.\]
For $\eps<1$, it follows that $\norm{\C}^2\le4\norm{\A}^2$, so that $\norm{\C^\top\C-\B^\top\B}\le\frac{\eps}{4}\norm{\A}^2$. 
Hence, $\norm{\A^\top\A-\B^\top\B}\le\eps\norm{\A}^2$. 

If all nonzero entries of $\A$ are bounded by some polynomial in $n$, then each entry of $\C$ can be written as $\left(1+\frac{\eps}{6}\right)^m$ for some $m=\O{\frac{1}{\eps}\log n}$. 
Since storing the value of $m$ requires $\log\log n+\log\frac{1}{\eps}$ bits, then each entry of $\C$ can be succinctly expressed in $\log\log n+\log\frac{1}{\eps}$ bits. 
\matrixmult{} stores $\O{\frac{1}{\eps^2}\log n}$ rows, with high probability, each with dimension $d$, so the total bit complexity is $\O{\frac{d}{\eps^2}\log n\left(\log\log n+\log\frac{1}{\eps}\right)}$.
\end{proof}

\subsection{Lower Bounds for Covariance Approximation}
To show a lower bound for the covariance matrix approximation problem in the sliding window model, we consider the following variant of the \indexcc{} problem. 
For any positive integer $n$, suppose the first player Alice is given a string $S\in\{0,1\}^{n}$ chosen uniformly at random, while the second player Bob is given an index $m\in[n]$ chosen uniformly at random. 
Alice sends a message to Bob, who must output $S[m]$ with probability at least $\frac{2}{3}$.
We also use $R^\rightarrow_{\mu,\delta}(\indexcc)$ to denote the minimum communication of a protocol that sends a single message from Alice to Bob for solving \indexcc{} with probability at least $1-\delta$, where the probability is taken over both the input distribution $\mu$ and the randomness of the protocol. 
\begin{lemma}\cite{MiltersenNSW95}
\lemlab{lem:cc:index}
Let $\mu$ be the uniform distribution on $\{0,1\}^n\times [n]$. 
Then $R^\rightarrow_{\mu,\delta}(\indexcc)=\Omega(n)$.
\end{lemma}
We first give a lower bound for the covariance matrix approximation problem in the streaming model to build intuition. 
In this setting, Alice will convert her string into a matrix $\A=\left[\M|\bE\right]$. 
The submatrix $\M$ will encode the characters of her string while the submatrix $\bE$ will consist of a number of elementary columns. 
Hence, $\A^\top\A$ will consist of many cross-products between $\M$ and $\bE^\top$ that will inform Bob about the characters of the string. 
In other words, if Bob obtains a good approximation of $\A^\top\A$, Bob can determine a large fraction of the string. 
\begin{theorem}
\thmlab{thm:lb:mm:stream}
Let $\A$ be a $n\times d$ matrix and $\eps>0$. 
Any one-pass streaming algorithm that returns a matrix $\B$ such that $\norm{\A^\top\A-\B^\top\B}_F\le\eps\norm{\A}_F^2$ with probability at least $\frac{8}{9}$ requires $\Omega\left(\frac{d}{\eps^2}\right)$ bits of space.
\end{theorem}
\begin{proof}
Suppose Alice receives a string $S\in\{0,1\}^{d/324\eps^2}$ chosen uniformly at random and creates a $\frac{1}{324\eps^2}\times d$ matrix $\M$ by setting each entry 
\[
\M_{i,j}=
\begin{cases}
18\eps & \text{if}~S\left[(i-1)d+j\right]=1\\
-18 \eps & \text{if}~S\left[(i-1)d+j\right]=0.
\end{cases}
\]

Let $\e_i$ be the elementary column vector with a one in the $i\th$ position and zeroes elsewhere. 
Alice creates a matrix $\bE$ that has $324\eps^2 d$ instances of $\e_1$, followed by $324\eps^2 d$ instances of $\e_2$, and so forth, for each of the $\frac{1}{324\eps^2}$ elementary column vectors. 
Alice then creates a $\frac{1}{324\eps^2}\times 2d$ matrix $\A=\begin{bmatrix}\M & \bE\end{bmatrix}$. 
Intuitively, the entries of $\M^\top\bE$ and $\bE^\top\M$ in $\A^\top\A$ reveal the entries of $\M$, in which Alice has encoded characters of $S$. 
Alice sends each row of $\A$ to the covariance matrix approximation algorithm and then passes the state of the algorithm to Bob. 

Bob uses the state of the algorithm to compute a matrix $\B$. 
Given an index $m\in\left[\frac{d}{324\eps^2}\right]$ chosen uniformly at random, Bob sets integers $(y-1)d+z=m$, where $1\le y\le\frac{1}{324\eps^2}$ and $1\le z\le d$, and deduces that 
\[
S[m]=1 ~\text{if}~ \A_{y,z}=18\eps \quad \text{or} \quad S[m]=0~\text{if}~\A_{y,z}=-18\eps. 
\]

To compute $\A_{y,z}$, Bob computes $\B^\top\B$ and then looks at the entries 
\[(\B^\top\B)_{z,j}~\text{for all } j=n+(y-1)(324\eps^2 d)+b,\] 
where $1\le b\le 324\eps^2 d$, and outputs $S[m]=1$ if the majority of these entries are positive and $S[m]=0$ if the majority of these entries are negative.    

\begin{claim}
\clmlab{clm:bob}
Let $\A$, $\B$, and $S$ be as defined above. Then if $\norm{\A^\top\A-\B^\top\B}\le\eps\norm{\A}_F^2$, then Bob can identify a large fraction of the indices $S[i]$. 
\end{claim}
\begin{proof}
First note that each column in $\A$ is a unit vector so $\norm{\A}_F^2=2d$. 
Let $\c_i$ represent the $i\th$ column of $\A$ so that $(\A^\top\A)_{i,j}=\langle c_i,c_j\rangle$. 

In particular, if $1\le z\le d$ and $j=d+(y-1)(324\eps^2 d)+b$ for some integers $1\le y\le\frac{1}{324\eps^2}$ and $1\le b\le 324\eps^2 d$, then
\[(\A^\top\A)_{j,z}=(\A^\top\A)_{z,j}=\langle c_z,c_j\rangle=\A_{y,z}=\pm 18\eps.\]
Since there are $d$ total such indices $j$, then the total contribution of these entries $(\A^\top\A)_{j,z}$ and $(\A^\top\A)_{z,j}$ to the Frobenius norm of $\A^\top\A$ is $18\sqrt{2}\eps d$. 
Hence, for $\norm{\A^\top\A-\B^\top\B}\le\eps\norm{\A}_F^2\le2\eps d$, more than $\frac{8}{9}$ of the entries in $(\B^\top\B)_{j,z}$ and $(\B^\top\B)_{z,j}$ must have the same sign as $(\A^\top\A)_{j,z}$ and $(\A^\top\A)_{z,j}$ for $1\le z\le d$ and $j=d+(y-1)(324\eps^2 d)+b$, where $1\le y\le\frac{1}{324\eps^2}$ and $1\le b\le324\eps^2 d$. 
Intuitively, there can only be a small number of positions in $\B^\top\B$ that differ in sign with the corresponding positions of $\M^\top\bE$ or $\bE^\top\M$. 
This allows Bob to recover a large fraction of the indices of $S$ and we get the claim.  
\end{proof}

We call an entry in $\B^\top\B$ \emph{bad} if it does not have the same sign as the corresponding entry in $\A^\top\A$, so that at most $\frac{1}{9}d^2$ entries in $(\B^\top\B)_{i,j}$ can be bad, for $1\le i\le d$ and $j=d+(y-1)(324\eps^2 d)+b$ for some integers $1\le y\le\frac{1}{324\eps^2}$ and $1\le b\le 324\eps^2 d$. 
Since each column vector is repeated $324\eps^2 d$ times, the majority of the entries in the set $\{\B^\top\B\}_{z,j}$ is bad only if at least $162\eps^2 d$ entries are bad for a fixed $z$ across $j=d+(y-1)(324\eps^2 d)+b$, where $1\le b\le 324\eps^2 d$. 
Thus, Bob can err on at most $\frac{\frac{1}{9}d^2}{162\eps^2 d}=\frac{d}{1458\eps^2}$ of the $\frac{d}{324\eps^2}$ entries in $\A$. 
The probability that Bob fails to correctly compute $S[m]$ is at most $\frac{324\eps^2}{1458\eps^2}=\frac{2}{9}$, conditioned on the algorithm correctly giving a matrix $\B$ such that $\norm{\A^\top\A-\B^\top\B}\le\eps\norm{\A}_F^2$. 
Hence, the overall probability that Bob succeeds is at least $\frac{8}{9}-\frac{2}{9}=\frac{2}{3}$, so by \lemref{lem:cc:index}, any covariance matrix approximation algorithm that succeeds with probability at least $\frac{8}{9}$ must use $\Omega\left(\frac{d}{\eps^2}\right)$ bits of space.  
\end{proof}
We now give a lower bound for the covariance matrix approximation problem in the sliding window model. 
The argument follows similarly from \thmref{thm:lb:mm:stream}, but we show Alice and Bob would be able to communicate a longer string if they were able to do covariance matrix approximation in the sliding window model. 
Alice breaks the input string $S$ into $\log d$ substrings $S_1,\ldots,S_{\log d}$. 
She uses $S_i$ to create a matrix $\A_i=\left[\M_i|\bE_i\right]$ as before. 
However, the magnitude of the entries in each $\A_i$ are geometrically decreasing as $i$ increases. 
Hence, Bob can deduce the sign of any entry in $\A_k$ of interest by expiring the rows of all matrices $\A_j$ with $j<k$ so that the entries of $\A_k$ dominates the remaining entries. 
The rest of the argument follows as before, showing that $\A_k^\top\A_k$ encodes information about a large fraction of the characters of $S_k$. 
Since he can do this for any $k$ of interest, then Bob can determine a large fraction of the entire string $S$. 
\begin{theorem}
\thmlab{thm:lb:mm:sliding}
Let $\eps>0$ and $\A$ be a $n\times d$ matrix for $n=\frac{1}{72^2\eps^2}\log d$. 
Any sliding window algorithm that returns a matrix $\B$ such that $\norm{\A^\top\A-\B^\top\B}_F\le\eps\norm{\A}_F^2$ with probability at least $\frac{8}{9}$ requires $\Omega\left(\frac{d}{\eps^2}\log d\right)$ bits of space.
\end{theorem}
\begin{proof}
Suppose Alice receives a random string $S\in\{0,1\}^{\frac{d\log d}{72^2\eps^2}}$ chosen uniformly at random and creates matrices $\A^{(1)},\A^{(2)},\ldots,\A^{(\log d)}$ in the following manner. 
For each $1\le k \le \log d$, Alice initially creates the $\frac{1}{72^2\eps^2}\times d$ matrix $\M^{(k)}$ by setting each entry 
\[
\M_{i,j}^{(k)}=
\begin{cases}
	2^{-k+\log d}\cdot72\eps & \text{ if}~S\left[{72^2}{\eps^{-2}}(k-1)+(i-1)d+j\right]=1 \\
	-2^{-k+\log d}\cdot 72\eps & \text{ if}~S\left[{72^2}{\eps^{-2}}(k-1)+(i-1)d+j\right]=0.
\end{cases}
\] 
Let $\e_i$ be the elementary column vector with a one in the $i\th$ position and zeroes elsewhere. 
Alice creates a matrix $\bE^{(k)}$ that has $72^2\eps^2 d$ instances of $2^{-k+\log d}\e_1$, followed by $72^2\eps^2 d$ instances of $2^{-k+\log d}\e_2$, and so forth, for each of the $\frac{1}{72^2\eps^2}$ elementary column vectors. 
Alice then creates a $\frac{1}{72^2\eps^2}\times 2d$ matrix $\A^{(k)}=\begin{bmatrix}\M^{(k)} & \bE^{(k)} \end{bmatrix}$.  
Alice then sets 
\[\M=\begin{pmatrix} \A^{(1)} \\ \A^{(2)} \\ \vdots \\ \A^{(\log d)} \end{pmatrix} \in \set{0,1}^{\frac{\log d}{72^2 \eps^2}\times d}.\]  
Alice sends each row of $\M$ to the covariance matrix approximation algorithm and passes the state of the algorithm to Bob. 

For an index $m\in\left[\frac{d\log d}{72^2\eps^2}\right]$ chosen uniformly at random, let $1\le k\le\log d$ be the integer such that 
\[\frac{d(k-1)}{72^2\eps^2} < m\le \frac{dk}{72^2\eps^2}.\]
 
Bob expires the rows of all matrices $\A^{(i)}$ for $i<k$ by inserting $\frac{1}{72^2\eps^2}(k-1)$ rows of all zeroes so that the matrix represented by the sliding window is 
\[\A:=
\begin{pmatrix} \A^{(k)} \\ \A^{(k+1)}\\ \vdots \\ \A^{(\log d)} \\ \mathbf{0} \end{pmatrix}, \]
where $\mathbf{0}$ represents a matrix of dimension $\ell \times d$ such that $\ell := \frac{1}{72^2\eps^2}(-k+1+\log d)$.
  
Bob then uses the state of the algorithm to compute a matrix $\B$. 
Recall that the entries of $\M^{(k)}$ are bigger than the sum of the corresponding entries in $\M^{(j)}$ for $j=k+1$ to $j=\log d$, since each $\M^{(j)}$ has entries that are geometrically decreasing as $j$ increases. 
Similarly, the entries of $\bE^{(k)}$ are larger than the sum of the corresponding entries in $\bE^{(j)}$ for $j=k+1$ to $j=\log d$. 
Thus, the entries of $\A^\top\A$ that correspond to $\sum_{k}^{\log d}(\M^{(j)})^\top\bE^{(j)}$ or $\sum_{k}^{\log d}(\bE^{(j)})^\top\M^{(j)}$ are dominated by the values of $(\M^{(k)})^\top\bE^{(k)}$ or $(\bE^{(k)})^\top\M^{(k)}$ respectively, so Bob can use the sign of each entry in $\B^\top\B$ to deduce values in $S$, similar to the proof of \clmref{clm:bob}. 

We have that  $\norm{\A^{(i)}}_F^2 = \frac{2d^3}{2^{2i}}$ because every column of $\A^{(i)}$ has squared norm $\frac{d^2}{2^{2i}}$. Thus the Frobenius norm of $\A$ is at most 
\[\norm{\A}_F^2 = \sum_{i=k}^{\log d}\frac{2d^3}{2^{2i}}\le\frac{4d^3}{2^{2k}}.\]
 
On the other hand, if $1\le z\le d$ and $j=d+ 72^2\eps^2 d(y-1)+b$ for some integers $1\le y\le\frac{1}{72^2\eps^2}$ and $1\le b\le 72^2\eps^2 d$, then
\[(\A_k^\top\A_k)_{j,z}=\left((\A^{(k)})^\top\A^{(k)}\right)_{z,j}=\pm\frac{72d^2}{2^{2k}}\eps.\]
Note that each entry $(\A^\top\A)_{j,z}$ has the same sign as the corresponding entry $((\A^{(k)})^\top\A^{(k)})_{j,z}$ since
\[\left|\sum_{i=k+1}^{\log d}\left((\A^{(k)})^\top\A^{(i)}\right)_{j,z}\right|\le\frac{36d^2}{2^{2k}}\eps.\]
We call an entry $(j,z)$ in $\B^\top\B$, with $1\le y\le\frac{1}{72^2\eps^2}$ and $1\le b\le 72^2\eps^2 d$, \emph{bad} if $|(\B^\top\B)_{j,z}-(\A^\top\A)_{j,z}|\ge\frac{36d^2}{2^{2k}}\eps$. 
Since $\norm{\A}_F^2\le\frac{4d^3}{2^{2k}}$, any covariance matrix approximation algorithm that produces $\B$ with $\norm{\A^\top\A-\B^\top\B}_F\le\eps\norm{\A}_F^2$ can have at most $\frac{1}{9}d^2$ bad entries. 

Given this, Bob uses $m$ to set integers $y,z$ so that $m=\left(\frac{d}{72^2\eps^2}\right)(k-1)+(y-1)d+z$, where $1\le y\le\frac{1}{72^2\eps^2}$ and $1\le z\le d$, and deduces that $S[m]=1$ if $\A_{y,z}>0$ or $S[m]=0$ if $\A_{y,z}<0$. 
Bob can look at the entries $(\B^\top\B)_{z,j}$ for all $j=d+(72\eps)^2 n(y-1)+b$, where $1\le b\le (72\eps)^2 d$, and output $S[m]=1$ if the majority of these entries are positive and $S[m]=0$ if the majority of these entries are negative. 
Since the number of bad entries in $\B^\top\B$ is bounded by $\frac{1}{9}d^2$, by similar reasoning to the proof of \thmref{thm:lb:mm:stream}, the probability that Bob fails to correctly compute $S[m]$ is at most $\frac{2}{9}$, conditioned on the algorithm correctly giving a matrix $\B$ such that $\norm{\A^\top\A-\B^\top\B}\le\eps\norm{\A}_F^2$. 
Hence, the overall probability that Bob succeeds is at least $\frac{8}{9}-\frac{2}{9}=\frac{2}{3}$, so by \lemref{lem:cc:index}, any covariance matrix approximation algorithm that succeeds with probability at least $\frac{8}{9}$ must use $\Omega\left(\frac{d}{\eps^2}\log d\right)$ bits of space. 
\end{proof}
